The asymptotic number of lattice zonotopes in a hypercube

We provide a sharp estimate for the asymptotic number of lattice zonotopes, inscribed in $[0,n ]^d$ when $n$ tends to infinity. Our estimate refines the logarithmic equivalent established by Barany, Bureaux, and Lund when the sum of the generators of the zonotope is prescribed. As we shall see, the exponential part of our estimate is composed of a polynomial of degree $d$ in $n^{1/(d+1)}$, and involves Riemann's zeta function and its non-trivial zeros. %Our analysis is based on a mapping between sums of coprime numbers and Eulerian polynomials. We also analyze some combinatorial properties of lattice zonotopes. In particular, we provide the first moment of the polyhedral graph asymptotic diameter when $n$ goes to infinity.

==> Parties/2eulerian_poly.tex <==

The proof of Theorem \ref{theorem_1},  as it is the generalization of the result from \cite{Bureaux:polygons}, surprisingly follows the same framework, taking integral representation the integral through Mellin transform. It will lead to estimating the generating function near $\ttheta = 0$ using the utmost-left propagation of the integration contour of the transform. It turns out this method is possible thanks to the link between Eulerian polynomials and harmonic sums over primitive vectors. \medskip 

Let be $\aalpha \in \N^d$, $\un = (1,...,1)$, and $t > 0$, and denote $\text{int}(\R^d_{+})$ the interior of $\R^d_{+}$, the point in this section is to study the sum $S_{\aalpha} (e^{-t})$ that is

$$S_{\aalpha} (e^{-t}) = \sum_{\vv \in \P_{d+} \cap \text{int}(\R^d_{+})} \vv^{\aalpha} e^{ - t \un \cdot \vv} = \sum_{n = 1}^{+ \infty} \left( \sum_{\vv \in \P_{d+}\cap \text{int}(\R^d_{+}), \: \un \cdot \vv = n } \vv^{\aalpha} \right) e^{ - t n} $$

The partial sums over the primitive vectors with  {\color{red}L1-norm equals $n$} are denoted $S_n(\boldsymbol{\alpha})$. \medskip

\begin{rem}
As $\aalpha$ can have zero coordinate, the product $\vv^{\aalpha}$ is not always defined over $\P_{d+}$. the sum therefore covers non-zero-coordinated-integer. Yet the reader can see it as a sum over all elements of $\P_{d+}$ with the convention $\vv^{\aalpha} =0$ if and only if $\vv$ has a zero coordinate.   
\end{rem}

% \emph{dit pourquoi c'est cool Mellin, propriete de sortir les harmonique hors de l'integral. Réponse : je ne sais pas si c'est utile d'appuyer sur ça alors que les rapports disent que c'est vraiment facile d'utiliser Mellin, et je refais la propriété d'harmonique proprement avec Fubini plus loin.}
Before the proposition is given, we introduce the routinely used Mellin transform which is the transform that maps the exponential onto the Gamma function, that holds for all $s$, with $\Re(s) >0$:  

$$ \Gamma(s) = \int_{0}^{+ \infty} e^{-t} t^{s - 1} dt.$$

For a given function $f$ and two numbers $a <b$ such that $\underset{x \rightarrow 0}{\lim}f(x) = O(x^a)$ and  $\underset{x \rightarrow + \infty}{\lim}f(x) = O(x^b)$, for all $s$ with $a< \Re(s) <b$, the Mellin transform of $f$ is defined as:  

$$ \mathcal{M}\left[f\left(e^{-t}\right)\right](s) = \int_0^{+\infty} f\left(e^{-t}\right)t^{s-1}dt.$$


\begin{prop}\label{proposition_eulerian}

For $t>0$ and $s \in \C$ with $\Re(s) > \un \cdot \aalpha + d$:


 \begin{align}
     \mathcal{M}\left[ S_{\aalpha}(e^{-t}) \right](s) = \frac{1}{\zeta(s - \aalpha \cdot \un )} \mathcal{M}\left[ \frac { \prod_{i = 1}^{d}  A_{\alpha_i}(e^{-t})}{(1-e^{-t}) ^{\aalpha \cdot \un + d}}  \right](s) ,
 \end{align}
 
 where $A_{\alpha_i}$ denotes the Eulerian polynomial of degree $\alpha_i$.
\end{prop}

\medskip

Eulerian polynomials were first described by Euler \cite{Euler} while studying the series form of $\frac{y e^x}{1 - y e^x}$ \cite{Euler}. We denote $A_n$ the $n$-th Eulerian polynomial using the recursive definition:

$$\left\{ \begin{array}{l}
       A_0(y) = y,\text{ and} \\
       A_n(y) = \sum_{m= 0}^n A(n,m)y^{n-m}.
\end{array} \right.$$

Hence the first Eulerian polynomials are $A_1(y) = y, \; A_2(y) = y^2 + y,$ and $ A_3(y) = y^3 + 4 y^2 + y$. In particular, they satisfy the relation:

\begin{align}\label{eulerien_poly}
    \sum_{k=1}^\infty k^n y^{k}  &= \frac{ A_n (y)}{(1-y)^{n+1}}.
\end{align}

$$  
$$



\begin{lem}\label{lem_eulerian_sum_notation} 
For any complex number $y$ with $|y| < 1$, 
\begin{align}\label{relation_lem_eulerian}
    \sum_{k \geq 0} k^{\un \cdot \aalpha} S_{\aalpha} (y^k) =  \frac { \prod_{i = 1}^{d}  A_{\alpha_i}(y)}{(1-y) ^{\aalpha \cdot \un + d}} .
\end{align} 
\end{lem}

\begin{proof}

This relation relies on the partition $\N_+^r =\bigcup_{k \geq 0} \left\{ kp, p \in \mathbb{P}^r_+ \right\}$ and the definition of Eulerian polynomials. The left term can be written as: 

$$ \sum_{k \geq 0 } k^{\un \cdot \aalpha}  S_{\aalpha} (y^k) = \sum_{k \geq 0} \sum_{n \geq 1} \left(\sum_{\substack{ \vv \in \P_{d+} \cap \text{int}(\R^d_{+}) \\   \un \cdot \vv = n }}(k \vv)^{\aalpha}(y)^{k \un \cdot \vv} \right)$$ 

We recognize the set of summation to be the partition previously mentioned. Therefore, for $|y| < 1$, the term $\vv^{\aalpha} y^{\un \cdot \vv}$ implies the absolute convergence of this sum. Hence we can use Fubini-Tonelli theorem to inverse the sums, and the relation (\ref{eulerien_poly}) concludes the proof.

$$ \sum_{\substack{ \vv \in \N^d \cap \text{int}(\R^d_{+})} } \vv ^{\aalpha} y^{\vv}   = \prod_{i = 1}^{d} \left( \sum_{v_i \geq 1} v_i^{\alpha_i} y^{v_i} \right)  = \frac { \prod_{i = 1}^{d}  A_{\alpha_i}(y)}{(1-y) ^{\aalpha \cdot \un + d}}.  $$


\end{proof}


The $n^{th}$ Eulerian polynomial is of degree $n$ except for $A_0(y) = y$ and has no constant term which causes the degree of $\prod_{i = 1}^{d}  A_{\alpha_i}(y)$ to be no more than $\aalpha \cdot \un + d$ (which is achieved for $\aalpha = \textbf{0}$).  The $\aalpha$ of the sums under study in this paper are $\textbf{0}$, $(1,0..,0)$, and $(2,0...,0)$, and the product of polynomials, therefore equals $y^{d}$, $y^{d}$, or $y^{d+1}+ y^{d}$.\\


Note that $S_n(\boldsymbol{\alpha})$ is the sum of a power function over the primitive points contained in the hypersurface of the dilates of the $(r-1)$-dimensional standard simplex. It is noteworthy that the number of such points has been computed in \cite{DezaPournin:primitivepoint}.   \\


\begin{proof}[Proof of the proposition]

Under the condition $ \Re(s) > \aalpha \cdot \un + d - 1$, the Mellin transform of the sum (\ref{relation_lem_eulerian}) is defined. This condition ensures that {\tiny$\sup_{\Re(s) > \aalpha \cdot \un + d - 1} \sum_{k \geq 0} |\frac{k^{\aalpha \cdot \un}}{k^s} |$} is bounded, hence we can apply Fubini's theorem with the change of variable $t' = kt$  and we have:

$$ \int_0^{+\infty} \sum_{k \geq 0 } k^{\aalpha \cdot \un} S_{\aalpha}(e^{-kt}) t^{s-1} d t= \zeta(s-\aalpha\cdot \un) \: \mathcal{M}\left[ S_{\aalpha}(e^{-t}) \right](s).$$


These holomorphic functions being defined and equal on $\Re(s) > \aalpha \cdot \un + d - 1$, we can extend it to its meromorphic continuation on $\C$. We replace the left term using Lemma \ref{lem_eulerian_sum_notation} and get the proposition.

\end{proof}


The Mellin transform is widely used to estimate asymptotic behaviors using its correspondence with the poles of the transformed function, as we will do in next subsection (and as it is done in \cite{Bodini:polyomino} and \cite{Bureaux:polygons}).  Proposition \ref{proposition_eulerian} makes it possible to compute the asymptotic equivalent of any of the sums $S_{\aalpha}(y) $ near $y =1$. 




%%%%%% ON VA TOUT SUPPRIMER CE QUI EST EN DESSOUS




% \subsection{Riemann's non trivial zeros challenge, with the example \texorpdfstring{$\sum_{ \protect\substack{ p < n \\  p \wedge n = 1 }}\protect p^2$}{TEXT} }

% We use this subsection to detail more specifically the asymptotic development of an expression using utmost-left propagation of the integration contour in the Mellin inversion formula, as we will encounter it multiple times. The reader that well knows this method can carry on to next section. Riemann's $\zeta$ function's non-trivial zeros intervenes in it, we will use the integral of \cite{Bureaux:polygons} to manage all the zeros in the critical strip with an integral, but we could also write a sum over all non-trivial zeros. This term is numerically discussed in the Section \ref{numerical_discu}. 

% \begin{prop}
% We denote the contour $\gamma = \gamma_{\text{right}}\cup \gamma_{\text{left}}$, with $\gamma_\text{right} = 3 - \frac{A}{\log(2 + |t|)} +it$ and $\gamma_\text{left} = 2 + \frac{A}{\log(2 + |t|)}+it $ as $t$ runs from $-\infty$ to $+\infty$, with $A >0$ such that $\gamma$ surrounds all the zeros in the critical strip of $\zeta(s-2)$. \\

% Hereafter we will denote $$I_\text{crit} = \frac{1}{2i\pi} \int_\gamma  \mathcal{M}[\sum_{n \geq 1 } S_n (2, 0) e^{-  n t}](s) t^{-s} d s$$,\\

% We have for all $t>0$:

% \begin{align}
%      \sum_{n \geq 1 } S_n (2, 0) e^{-  n t} = \frac{2}{\zeta(2) t^{4}} + I_\text{crit}(t) + \frac{1}{3 t^2} - \frac{1}{90 \zeta'(-1)}\log(t)  + \underset{t \rightarrow 0}{O}(t^{1/2}).
% \end{align}

% \end{prop}

% \begin{proof}
% We take the general set of sums  $\left(\sum_{\substack{ p < n \\  p \wedge n = 1 }} p^i \right)_{i \geq 0}$.\\
% As $p \wedge n = 1$ being equivalent to $p \wedge (n-p) = 1$, those sums can be rewritten as $\sum_{ \substack{ p +q  = n \\  p \wedge q = 1 }} p^i = S_n(i,0)$.\\
% We fix $i = 2$. Applying Lemma \ref{lem_eulerian_sum_notation}, we have:

% \begin{align*}
%     \sum_{k \geq 0 } k^{2} \sum_{n \geq 1 } S_n (2, 0) e^{- k n t} &= \frac{A_0(e^{-t})  A_2 (e^{-t})}{(1-e^{-t})^{4}}\\
%     &= (e^{-3 t} + e^{-2t}) \sum_{k \geq 0} \binom{k+3}{3} e^{-k t}. 
% \end{align*}


% For $t >0, s >1 $, we have the following Mellin transform: 

% \begin{align*}
%     \mathcal{M} \left[ \sum_{n \geq 1 } S_n (2, 0) e^{-  n t}\right] (s) &= \frac{1}{\zeta(s-2)}\left(  \sum_{k \geq 1} \frac{\binom{k+1}{3} + \binom{ k }{3}}{k^s}  \Gamma(s)\right)\\
%     &= \frac{2 \zeta(s-3) - 3 \zeta(s-2) + \zeta(s-1)}{6 \zeta(s-2)}\Gamma(s) .
% \end{align*}


% Therefore we have, using  the Mellin inversion formula, for all $c > 4$ (to ensure $\sup_{s\in c+ i \R} \zeta(s-3) < \infty$):
 
%  $$ \sum_{n \geq 1 } S_n (2, 0) e^{-  n t} = \frac{1}{2i\pi} \int_{c- i\infty}^{c+ i\infty} \frac{2 \zeta(s-3) - 3 \zeta(s-2) + \zeta(s-1)}{6 \zeta(s-2)}\Gamma(s) t^{-s} d s. $$

% We use the residue theorem to shift the line of integration to the left as $s= 4$ is a location of a pole of the Mellin transform. It follows that, for all $c_1\in ]3, 4[$:

% $$ \sum_{n \geq 1 } S_n (2, 0) e^{-  n t} = \frac{2}{\zeta(2) t^{-4}} + \frac{1}{2i\pi} \int_{c_1- i\infty}^{c_1+ i\infty} \frac{2 \zeta(s-3) - 3 \zeta(s-2) + \zeta(s-1)}{6 \zeta(s-2)}\Gamma(s) t^{-s} d s.$$

% The remaining poles of the Mellin transform are the double pole at $s = 0$, and simple ones at $s=0$ and at the non-trivial zeros of $\zeta(s-2)$,  which are in the critic strip $2<\Re(z)<3$, and in the left side of the complex domain. \\

% Now consider the contour $\gamma$ as described in the proposition. The existence of $A$, such that $\gamma$ surrounds all the zeros of $\zeta(s-2)$ in the critical strip is a consequence of Theorem 3.8 in \cite{Titchmarsh:riemann}.

% \begin{align}\label{riemann_crit_strip}
%     I_\text{crit}(t) = \frac{1}{2i\pi} \int_\gamma  \frac{2 \zeta(s-3) - 3 \zeta(s-2) + \zeta(s-1)}{6 \zeta(s-2)}\Gamma(s) t^{-s} d s.
% \end{align}

% For any $c_2 \in ]0,2[$, we have:

% $$ \sum_{n \geq 1 } S_n (2, 0) e^{-  n t} = \frac{2}{\zeta(2) t^{-4}} + I_\text{crit}(t) + \frac{1}{3 t^2} +  \frac{1}{2i\pi} \int_{c_2- i\infty}^{c_2+ i\infty} \frac{2 \zeta(s-3) - 3 \zeta(s-2) + \zeta(s-1)}{6 \zeta(s-2)}\Gamma(s) t^{-s} d s. $$

% Finally denoting $I_\text{err} (t) = \frac{1}{2i \pi}\int_{\frac{1}{2} - i\infty}^{\frac{1}{2}+i\infty} \frac{2 \zeta(s-3) - 3 \zeta(s-2) + \zeta(s-1)}{6 \zeta(s-2)}\Gamma(s) t^{-s} d s$, we have for $t>0$

% $$ \sum_{n \geq 1 } S_n (2, 0) e^{-  n t} = \frac{2}{\zeta(2) t^{4}} + I_\text{crit}(t) + \frac{1}{3 t^2} - \frac{1}{90 \zeta'(-1)}\log(t)  + I_\text{err}(t). $$

% The bounds over the order of $I_\text{crit}$ and $I_\text{err}$ are coming from Lemma 2.2 from \cite{Bureaux:polygons}.
% \end{proof}



% %% Anciennement:: $$\sum_{n \geq 0 } \sum_{\substack{ p \leq n \\  p \wedge n = 1 }} p^{2} e^{-n t}  = \frac{12}{ \pi^2 t^4} - \frac{2}{t} + O(1).$$

% \end{proof}

% (see \cite{Bodini:polyomino,Flajolet:AC,Gittenberger:hadmi}). In the following, the analysis of zonotopes will require to apply a Mellin transform on sums of coprime numbers. The following proposition is of primary importance in the sequel:
% \begin{prop}\label{property2}
% For $t> 0$, the Mellin transform of $\sum_{n \geq 1} S_n(\boldsymbol{\alpha}) e^{-n t}$ is 
% \begin{align}
%      \frac{1}{\zeta(s-j)} \left( \sum_{n = 0}^{j + r } b_{\boldsymbol{\alpha},n}  \sum_{k \geq 1} \frac{\binom{ k  + j + %r - n - 1}{j + r -1 }}{k^s} \Gamma(s)\right) .
%  \end{align} 
%  \end{prop}

% \begin{proof}


==> Parties/4h_admissibility.tex <==
%Modifications: 
%-intro : parallele avec Boltzman proba ? Il faut dire ce que c'est que la saddle point method. 
%- A, B, C, les matrices dérivées à changer 
%- Ajouter des noms mathematiques dans les lemmes
% remettre en valeur la section des eulerians sets (dans l'intro)


The saddle point method is suitable when the integrand is subject to a abrupt variation, with a major negligible part, and a small one that can be approximated by a Gaussian integral. It can be typically the case if the path along which a function is integrated passes close to a pole. In the 50's, Hayman defined a class of analytic complex functions $\sum_n a_n x^n$, called H-admissible functions, for which one can use this method to estimate the coefficients $a_n$ \cite{Hayman}. Since then, many extensions of this concept have been made. As we have here a $d$ dimensional space, we will use the work of Gittenberger and Mandlburger  \cite{Gittenberger:hadmi} that extends the H-admissible class for functions on $d$-dimensional spaces.\\

\begin{thm}\label{h-admissible}
The function $Zon: \C^d \rightarrow \C  $ is H-admissible on $\mathcal{R}=\{\textbf{\textit{x}} \in \R^d,  \forall i \:\: |x_i| < 1  \}$ in the sense of Gittenberger et Mandlburger \cite{Gittenberger:hadmi}.
\end{thm}


This theorem relies on five conditions that we will prove in what follows. In order to prove them, we use the following notation:

Recall that $\widetilde{\theta}_n = \left(\frac{2^{d-1} d \zeta(d +1)}{ \zeta(d) n} \right)^{\frac{1}{d+1}}$ is the solution of the saddle equation and denote $x_n = \exp(- \widetilde{\theta}_n )$ ($x_n \rightarrow 1$ as $n \rightarrow \infty$). To be H-admissible, a function needs to be approximately its Gaussian distribution (i.e. its logarithm is approximately its own Taylor expand) on a small area, and to be small enough on the remaining domain in the integral.\\

This area is defined as $\Delta (\widetilde{\theta}_n ):= \left\{ \boldsymbol{\theta} = (\theta_i)_{1 \leq i \leq d}, \forall i \:\: |\theta_i| < \widetilde{\theta}_n ^\alpha\right\}$ for $\alpha $ picked in $ ]1 + \frac{d}{3} ,1 + \frac{d}{2}[$ (this interval is determined in the following lemma). \\

Finally, $\textbf{a}(\textbf{\textit{x}}) = \left(a_i(\textbf{\textit{x}})\right)_{1 \leq i\leq d}$, $\textbf{B}(\textbf{\textit{x}}) = \left(B_{i,j}(\textbf{\textit{x}})\right)_{1 \leq i,j \leq d}$, and $\textbf{C}(\textbf{\textit{x}}) = \left(C_{i,j,k}(\textbf{\textit{x}})\right)_{1 \leq i, j, k \leq d}$ respectively stand for the sets of the first, second, and third order partial derivative of the logarithm of $Zon(\textbf{\textit{x}})$.


\begin{proof}
The first and the third points directly follow the asymptotic equivalent we have in (\ref{equivalent_B}). As for the second point, it is an outcome of Lemma \ref{condition2}.
\end{proof}
